Just Zoom In: Cross-View Geo-Localization via Autoregressive Zooming

Cross-view geo-localization (CVGL) estimates a camera's location by matching a street-view image to geo-referenced overhead imagery, enabling GPS-denied localization and navigation. Existing methods almost universally formulate CVGL as an image-retrieval problem in a contrastively trained embedding space. This ties performance to large batches and hard negative mining, and it ignores both the geometric structure of maps and the coverage mismatch between street-view and overhead imagery. In particular, salient landmarks visible from the street view can fall outside a fixed satellite crop, making retrieval targets ambiguous and limiting explicit spatial inference over the map. We propose Just Zoom In, an alternative formulation that performs CVGL via autoregressive zooming over a city-scale overhead map. Starting from a coarse satellite view, the model takes a short sequence of zoom-in decisions to select a terminal satellite cell at a target resolution, without contrastive losses or hard negative mining. We further introduce a realistic benchmark with crowd-sourced street views and high-resolution satellite imagery that reflects real capture conditions. On this benchmark, Just Zoom In achieves state-of-the-art performance, improving Recall@1 within 50 m by 5.5% and Recall@1 within 100 m by 9.6% over the strongest contrastive-retrieval baseline. These results demonstrate the effectiveness of sequential coarse-to-fine spatial reasoning for cross-view geo-localization.

==> tables/bb_comp.tex <==
\begin{table}
\caption{\textbf{Comparison of different frozen vision backbones.} We evaluate different frozen vision encoder backbones for our autoregressive geo-localization task. Overall, DINOv2 achieves the strongest performance, outperforming more recent architectures.}

  \label{tab:backbone_comp}
  \centering
  \begin{tabular}{l c c c}
    \toprule
    \textbf{Method} & \textbf{R@40m} $\uparrow$ & \textbf{R@50m} $\uparrow$ & \textbf{R@100m} $\uparrow$ \\
    \midrule
    SigLIP2-B~\cite{tschannen2025siglip2}  & 28.42 & 33.23 & 45.43\\
    DINOv3-B~\cite{simeoni2025dinov3}   & 63.88 & 69.44 & 79.74\\
    \midrule
    DINOv2-B~\cite{Oquab2023dinov2}   & \textbf{64.13} & \textbf{69.65} & \textbf{79.95}\\
    \bottomrule
  \end{tabular}
\end{table}


==> tables/ft_comp.tex <==
\begin{table}
\caption{\textbf{Impact of partial backbone fine-tuning.} We evaluate different degrees of layer freezing in the vision encoder for our autoregressive geo-localization task. Overall, unfreezing the last 4 layers yields the best performance, outperforming both fully frozen and fully fine-tuned configurations.}

  \label{tab:froze_comp}
  \centering
  \begin{tabular}{l c c c}
    \toprule
    \textbf{Method} & \textbf{R@40m} $\uparrow$ & \textbf{R@50m} $\uparrow$ & \textbf{R@100m} $\uparrow$ \\
    \midrule
    Fully Frozen  & 58.79 & 64.66 & 76.51\\
    Last 4 Layers & \textbf{66.98} & \textbf{72.25} & \textbf{83.08}\\
    Last 6 Layers & 65.69 & 70.64 & 82.56\\
    All Layers    & 59.45 & 64.31 & 74.78\\
    \bottomrule
  \end{tabular}
\end{table}

==> tables/ground_handling_comp.tex <==
\begin{table}
\caption{\textbf{Comparison of different ground image handling strategies.} We evaluate different preprocessing and embedding strategies for handling ground images in our geo-localization setup.}
\label{tab:ground_image_handling}
\centering
\begin{tabular}{l c c c}
  \toprule
  \textbf{Method} & \textbf{R@40m} $\uparrow$ & \textbf{R@50m} $\uparrow$ & \textbf{R@100m} $\uparrow$ \\
  \midrule
  Resize & 54.85 & 61.25 & 73.38 \\
    Split  & \textbf{67.23} & 71.66 & 82.56 \\
  Split \& Avg. & 66.98 & \textbf{72.25} & \textbf{83.08} \\
  \bottomrule
\end{tabular}
\end{table}

